Diffusion-Based Offline RL for Improved Decision-Making in Augmented ARC Task

Effective long-term strategies enable AI systems to navigate complex environments by making sequential decisions over extended horizons. Similarly, reinforcement learning (RL) agents optimize decisions across sequences to maximize rewards, even without immediate feedback. To verify that Latent Diffusion-Constrained Q-learning (LDCQ), a prominent diffusion-based offline RL method, demonstrates strong reasoning abilities in multi-step decision-making, we aimed to evaluate its performance on the Abstraction and Reasoning Corpus (ARC). However, applying offline RL methodologies to enhance strategic reasoning in AI for solving tasks in ARC is challenging due to the lack of sufficient experience data in the ARC training set. To address this limitation, we introduce an augmented offline RL dataset for ARC, called Synthesized Offline Learning Data for Abstraction and Reasoning (SOLAR), along with the SOLAR-Generator, which generates diverse trajectory data based on predefined rules. SOLAR enables the application of offline RL methods by offering sufficient experience data. We synthesized SOLAR for a simple task and used it to train an agent with the LDCQ method. Our experiments demonstrate the effectiveness of the offline RL approach on a simple ARC task, showing the agent's ability to make multi-step sequential decisions and correctly identify answer states. These results highlight the potential of the offline RL approach to enhance AI's strategic reasoning capabilities.

==> 99_acknowledgements.tex <==
\subsubsection*{Acknowledgements}
This work was supported by the IITP (RS-2023-00216011, RS-2024-00445087, No.~2019-0-01842) and the NRF (RS-2024-00451162) grants funded by the Ministry of Science and ICT, Korea. GPUs were supported by AICA and GIST SCENT. 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> not_used/4.1_task_explanation.tex <==
% \section{Synthesizing SOLAR for a simple task}

%%  Experiment와 result의 내용을 분리해서 각각 하나의 큰 section으로 변경했습니다.

% \label{Sec:SOLAR_for_single_task}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figure/data_ex_v4.pdf}
%   \caption{Synthesizing SOLAR for a simple task: The golden standard trajectory contains the shortest path to solve the problem. The non-optimal trajectory branches off at a random step within the standard trajectory, performing random operations such as \texttt{Rotate}, \texttt{Flip}, or \texttt{Copy} \& \texttt{Paste}, and then \texttt{Submit} after a certain number of steps.}
%   \label{fig:task}
% \end{figure}

% We construct the dataset to include trajectories where the model predicts the \texttt{Submit} operation at the answer state (golden standard), fails to reach the goal (non-optimal), or reaches the goal but performs other operations instead of \texttt{Submit} (non-optimal). To focus solely on evaluating the planning abilities of the LDCQ method, we designed a simple task with only 2 to 3 straightforward selection options, allowing for the assessment of the AI's planning ability by sequentially combining operations. As shown in Figure~\ref{fig:task}, the golden standard trajectory for this task consists of 5 steps: (1) \texttt{ResizeGrid} to make the grid 2 times longer vertically, (2) \texttt{CopyO} to copy the upper half of the current grid, as it matches the input grid, (3) \texttt{Paste} to apply it to the lower half of the grid, (4) \texttt{FlipV} to vertically flip the upper half of the current grid, and (5) \texttt{Submit}, as it reaches the answer state.
% % We construct the dataset to include trajectories where the model predict \texttt{Submit} operation at the answer state (golden standard), fails to reach the goal (non-optimal), or reaches the goal but performs other operations instead of \texttt{Submit} (non-optimal). After synthesizing SOLAR, we train AI with LDCQ method and evaluate.

% % We designed a simple task where the selection is relatively straightforward, allowing us to focus solely on evaluating the planning abilities of LDCQ method by sequentially combining operations. As shown in Figure~\ref{fig:task}, the golden standard trajectory for the task consists of 5 steps, as follows: (1) \texttt{ResizeGrid} with 2 times longer in vertically. (2) \texttt{CopyO}, copy a uppder half of current grid (because it matches the input grid) (3) \texttt{Paste} it to the below half of the grid. (4) \texttt{FlipV}, vertically flip the  uppder half of current grid. (5) \texttt{Submit} because it is answer state.

% We included non-optimal trajectories to prevent the AI agent from simply following the operations in the data. In the non-optimal trajectories, the agent initially follows the golden standard trajectory but deviates at a random step to execute random actions for several steps. We constrained the random operations to \texttt{FlipV} (vertical flip), \texttt{FlipH} (horizontal flip), \texttt{Rotate90} (counterclockwise rotation), \texttt{Rotate270} (clockwise rotation), and \texttt{CopyO} (updating the clipboard with the selected area). For selection, we constrained it to either 2 options (upper half of the current grid or lower half of the current grid) or 3 options (upper half, lower half, or the whole grid), with 2 options for \texttt{Rotate90}, \texttt{Rotate270}, and \texttt{CopyO}, and 3 options for the others. When \texttt{CopyO} is selected, \texttt{Paste} is forced onto the other possible selection option. The non-optimal trajectory contains approximately 10 steps per episode, allowing the AI to learn about various actions in diverse states. For each problem pair, we generated one golden standard episode and 9 non-optimal episodes, totaling 5,000 episodes across 500 problem pairs. As a result, the training set was composed such that approximately 10\% of the total episodes included the \texttt{Submit} operation at the answer state.

% With SOLAR, rather than considering all possible actions in the broad action space, the model focuses on actions from the training data with some added variance. Thus, if the dataset includes meaningful operations and selections relevant to the task, the model can learn the transitions induced by these operations more effectively. To facilitate this, we restricted selections to three types of pattern: the upper half of gird, the lower half of grid and the entire grid, allowing the model to recognize operations on a pattern level. Operations were composed of pattern-level manipulations like \texttt{Rotate}, \texttt{Flip}, and \texttt{Copy} \& \texttt{Paste}.

% ARCLE has a very large state space, and actions can be combined in complex ways through operations and selections. LDCQ encodes both the state and the action taken at that state into a latent vector, making it dependent on the actions included in the training dataset. The state and action are encoded together into a latent space, and similar latents are generated through the diffusion model. Therefore, 





% ARCLE은 state가 매우 크고, operatoin과 selection으로 action을 매우 복잡하게 조합할 수 있다. LDCQ는 특정 state에서 행했던 action을 같이 latent로 인코딩하여 사용하기에 데이터셋에 포함돼 있는 action들에 의존적인이다. state와 action을 같이 latent로 인코딩하고 이와 유사한 latent를 diffusion model로 생성한다. 그렇기에 넓은 action space의 가능한 action들을 다 보는 것이 아니라 학습 데이터에 있는 action에서 variance가 추가된 것을 고려하는 것이다. 따라서 데이터셋을 구성할 때 task에 의미있는 operation과 selection을 많이 포함한다면 operation에 의한 trainsition에 대한 정보들을 모델이 더 잘 학습할 수 있을 것이라 생각했다. 그래서 selection은 직사각형 기준 위의 정사각형 pattern, 아래의 정사각형 pattern, grid 전체를 선택하는 세가지로 제한하여 pattern 단위의 opertaion임을 잘 인지하도록 했고, operation들은 pattern 단위에 적용되는 rotation, \texttt{flip}, \texttt{copy}\&\texttt{paste}들로 구성했다. 

% single task에 대해서 reasoning 능력을 보이기 위해서 어렵지 않은 task를 만들었다. 그림과 같이 input으로 주어진 정사각형 grid를 복사하여 뒤집어서 위아래로 긴 직사각형 grid를 만드는 task이다. ARCLE에서는 grid의 state를 변화하는데 필요한 action을 selection과 operation의 조합으로서 수행한다. 이번 연구에서는 순전히 LDCQ모델에서 operation을 연속적으로 조합하는 것을 통한 planning/reasoning 능력을 평가하기 위해서 selection의 선택은 비교적 쉬운 task를 만들었다. input grid를 하나의 패턴으로 간주하고 이 패턴에 다양한 operation들을 적용하도록 만들었다. 해당 task에 대해 정답까지 가장 빠르게 도달하는 trajectory와, 그 trajectory 중간중간에서 branch를 만들어서 해당 패턴에 대화 \texttt{roate}/\texttt{flip} 등 다양한 operation들을 random하게 수행하는 trajectory를 같이 만들어서 expert와 random이 섞여있는 데이터셋을 구성했다. 하나의 problem pair에 대해 1개의 expert episode, 4개의 random episode를 포함하여 총 1000개의 problem pair에 대해 5000개의 episode를 포함하는 데이터셋을 사용했다. evaluation에는 train set과 다른 random seed를 사용해서 만든 example pair와 problem을 이용했다. 

==> not_used/4.2_ARC.tex <==
% \subsection{Training LDCQ method with SOLAR}

%  이부분은 detail한 내용이 커서 Appendix A training detail의 표 위로 옮겼습니다.








%  we used a horizon length of 5 for encoding skill latent, meaning that the model plans and evaluates actions over a five-step lookahead. In ARCLE, after submitting the grid to receive a reward, the episode ends when the state matches the correct answer~\cite{lee2024arcle}. 만약 None padding이 없다면 무조건 다른 action들을 수행하다가 마지막에 Submit을 누르는 latent들만 존재하기에 정답 상태에서도 submit을 잘 누르지 못한다. To help the model efficiently recognize when the current state is the correct answer and that it needs to execute the \texttt{Submit} operation, we added a \texttt{None} padding after the \texttt{Submit} action. Thus, all segment trajectories were made to have a horizon of 5, and for segments that included a \texttt{Submit} action, we padded the remaining horizon with \texttt{None} operations until it was filled.
%  인코딩한 latent를 이용해서 500step의 diffusion step을 거쳐서 diffusion model을 학습시켰다. diffusion step은 sampling하는 latent에 얼마나 variance를 주는 지에 영향을 준다. diffusion step이 촘촘할수록 noise를 적용하는 정도가 작아진다. 이후 Q-Network를 학습시킬 때 variance를 추가하기 위해서 diffusion step을 추가적으로 적용해서 sampling하는데, diffusion step을 작게하거나, extra diffusion step을 많이 추가하면 sampling된 latent의 variance가 커진다. ARCLE에서는 이 variance가 너무 커지게 되면 operation이나 selection 선택시에 오류가 많이 발생하기에 diffusion step을 500으로 설정하여 최대한 selection 선택시의 오류를 줄이고자 했다. 
% we set the discount factor to 0.5, ensuring the model appropriately balances immediate and future rewards. discount factor를 크게 하면 미래에 더 큰 보상을 받을 수 있는 것을 고려하기에 sparse reward 환경에서도 reward를 받으려는 방향으로 planning한다는 장점이 있다. 하지만 ARC에서는 정답까지 도달하는데 걸리는 time step이 짧기에 discount factor가 클 필요가 없고 오히려 discount factor가 크다면 정답 state에서도 몇 step 더 수행하다가 submit하고 reward를 받는 것과의 기댓값 구별이 어려워 정답임에도 submit을 하지 않는 현상이 발생한다. 



==> table/result.tex <==
\begin{table}[htbp!]
\centering
\caption{Performance comparison between only diffusion sampling and with Q-function}
\label{tab:result}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\textbf{ }                & \textbf{Diffusion Sampling w/o Q-function}   & \textbf{Diffusion Sampling w/ Q-function  } \\ 
\midrule
reach the answer grid              &   -                 &  -\\ 
submit correct answer               & 12.0                 & 60.0\\ 


\bottomrule
\end{tabular}
}
\end{table}
